What External Knowledge is Preferred by LLMs? Characterizing and Exploring Chain of Evidence in Imperfect Context for Multi-Hop QA

Incorporating external knowledge has emerged as a promising way to mitigate outdated knowledge and hallucinations in LLM. However, external knowledge is often imperfect, encompassing substantial extraneous or even inaccurate content, which interferes with the LLM's utilization of useful knowledge in the context. This paper seeks to characterize the features of preferred external knowledge and perform empirical studies in imperfect contexts. Inspired by the chain of evidence (CoE), we characterize that the knowledge preferred by LLMs should maintain both relevance to the question and mutual support among the textual pieces. Accordingly, we propose a CoE discrimination approach and conduct a comparative analysis between CoE and Non-CoE samples across significance, deceptiveness, and robustness, revealing the LLM's preference for external knowledge that aligns with CoE features. Furthermore, we selected three representative tasks (RAG-based multi-hop QA, external knowledge poisoning and poisoning defense), along with corresponding SOTA or prevalent baselines. By integrating CoE features, the variants achieved significant improvements over the original baselines.

==> sec/3.Methodology.tex <==
\section{Methodology}
\label{sec:approach}

To investigate whether the theory of evidence chain completeness can be applied to real-world scenarios, we propose {\tool} and integrate it into RAG. 
The original RAG workflow retrieves multiple relevant knowledge snippets for a question using a search engine, then uses a reranking model to rank all knowledge snippets, and selects the top-k snippets as context input for LLMs.
% {\tool} replaces the ranking phase in the original RAG with a method that selects the minimal set of knowledge snippets covering a complete COE as context input for LLMs. 
Instead of using the ranking phase in RAG, {\tool} selects the minimal set of knowledge snippets that encompasses a complete COE as context input for LLMs. 
It consists of two phases: 1) \textbf{COE Identification}, which identifies the COE elements covered by each knowledge snippet; 2) \textbf{Minimal Coverage Search}, which finds the minimal set of knowledge snippets that covers the complete COE.

\subsection{COE Identification}
{\tool} first extracts COE elements from the question and then identifies them in each knowledge snippet.
Specifically, as shown in Figure \ref{fig:loopjudge}, {\tool} employs the same information extraction component from the pipeline to extract intent, keywords, and relations from the question.
Then, for each knowledge snippet, {\tool} utilizes the same completeness identification component from the pipeline to determine whether it contains these extracted elements, and records the judgment results. Finally, we obtain a set of judgments regarding intent, keywords, and relations for each knowledge snippet.


\subsection{Minimal Coverage Search}
After obtaining the judgement set, {\tool} searches for the minimal set of knowledge snippets that covers the complete COE.
The detailed algorithm process is shown in Algorithm \ref{alg:minimal_coverage}. 
First, {\tool} searches for knowledge snippets containing intent (i.e., evidence) and adds all evidence to the minimal set. 
Then, it searches for the logical chain supporting the evidence, (i.e., the keywords and relations contained in the query).
{\tool} begins by examining relation coverage. 
It first determines if the minimal set already contains all relations.
If there are uncovered relations, it searches the remaining knowledge snippets and adds those containing uncovered relations to the minimal set. 
 Then {\tool} proceeds to examine keyword coverage following the same process.
It first checks if the minimal set covers all keywords.
If uncovered keywords exist, it searches the remaining snippets for those containing these keywords.

{\tool} manages to search for the minimal set that completely covers all COE elements, ultimately outputting a set of knowledge snippets that covers the maximum number of COE elements, which serves as context input for the LLM.


\begin{algorithm}[t]
\caption{Minimal Coverage Search}
\footnotesize
\label{alg:minimal_coverage}
\KwIn{External knowledge list $EK$, 
Identified external knowledge list $IEK$, where each item contains Intent, Relations, and Keywords judgments}
\KwOut{
Set $S$ of minimal coverage external knowledge}
$S \leftarrow \emptyset$\;
\# Phase 1: Intent Coverage\;
\For{$i \leftarrow 0$ \KwTo $|IEK|-1$}{
    \If{$IE[i].Intent = \text{TRUE}$}{
        $S \leftarrow S \cup \{EK[i]\}$
    }
}
% \# Phase 2: Relation Coverage\;
% $R \leftarrow$ GetRelationPositions($IE$)\;
% \For{$pos \in R$}{
%     \If{$R[pos] \cap S = \emptyset$}{
%         $S \leftarrow S \cup \{R[pos][0]\}$
%     }
% }

% \# Phase 2: Relation Coverage\;
% $R_{uncovered} \leftarrow$ GetUncoveredRelations($IEK, S$)\;
% \For{$r \in R_{uncovered}$}{
%     $candidates \leftarrow$ FindKnowledgeWithRelation($IEK, r$)\;
%     \If{$candidates \neq \emptyset$}{
%         $S \leftarrow S \cup \{candidates[0]\}$
%     }
% }

\# Phase 2: Relation Coverage\;
$R_{uncovered} \leftarrow$ GetUncoveredRelations($IEK, S$)\;
\For{$r \in R_{uncovered}$}{
    \For{$i \leftarrow 0$ \KwTo $|IEK|-1$}{
        \If{$IEK[i].Relations[r] = \text{TRUE}$}{
            $S \leftarrow S \cup \{EK[i]\}$\;
            \textbf{break}\;
        }
    }
}

\# Phase 3: Keyword Coverage\;
$K_{uncovered} \leftarrow$ GetUncoveredKeywords($IEK, S$)\;
\For{$k \in K_{uncovered}$}{
    \For{$i \leftarrow 0$ \KwTo $|IEK|-1$}{
        \If{$IEK[i].Keywords[k] = \text{TRUE}$}{
            $S \leftarrow S \cup \{EK[i]\}$\;
            \textbf{break}\;
        }
    }
}
% \Return{Sort($S$)}\;
\Return{S}\;
\end{algorithm}

==> sec/4.experiment.tex <==
\section{Evaluation}
\label{sec:experiment}

\subsection{Research Questions}
Our evaluation mainly aims to answer the following research questions:

\textbf{RQ1:} Given correct retrieved information, how does question-oriented knowledge completeness affect the effectiveness of retrieval-augmented LLMs?
%我们这个不是chatbot，chatbot得有bing那种。

\textbf{RQ2:} How do retrieval-augmented LLMs comply with question-oriented knowledge completeness?

\textbf{RQ3:} How robust is question-oriented knowledge completeness when used as retrieved information?

\textbf{RQ4:} Can retrieving question-oriented knowledge completeness improve LLM response accuracy in real-world RAG scenarios?









==> sec/todo.tex <==
1.加上senp和wordp的示意图
2.information 和knowledge说法要统一，特别是irrelevant这些后面的表述
3. conflict 和incorrect要统一
4.RQ4  retrieval phase 还是 reranking phase
5. LLM 的名称要全文统一，文字和表
6. 以往的study是关于retrieve更多感觉，而不是rerank
7.还要加上一个风险是我们没有单独对每个元素的重要性进行评估。
8.我们的方法是retrival ，尽管是在rerank阶段
9.limitation 加上一点，retrieval不能用于所有rag场景，比如那种vector的场景
10. evidence piece, textual piece, knowledge piece用哪个

==> tab/RQ4.tex <==
\begin{table}[t] 
\large
  \caption{ LLMs' Accuracy (ACC) on baselines and {\tool}.}
  \label{tab:link_performance}
  
\resizebox{0.5\textwidth }{!}{
\begin{threeparttable}
\begin{tabular}{cc|ccccccccc}
\toprule
\multirow{2}{*}{\textbf{Scenarios}} &
\multirow{2}{*}{\textbf{Model}} &
  

  \multicolumn{4}{c}{\textbf{HotpotQA}} & &
  \multicolumn{4}{c}{\textbf{2WikiMultihopQA}}
  \\    \cline{3-6} \cline{8-11} 


     &
   &

   \multicolumn{1}{c}{\textit{\textbf{CoT\_SC}}} &
\multicolumn{1}{c}{\textit{\textbf{VE}}} &
  \multicolumn{1}{c}{\textit{\textbf{RAG}}} &
  \multicolumn{1}{c}{\textit{\textbf{{\tool}}}} & 
  &
  \multicolumn{1}{c}{\textit{\textbf{CoT\_SC}}} &
\multicolumn{1}{c}{\textit{\textbf{VE}}} &
  \multicolumn{1}{c}{\textit{\textbf{RAG}}} &
  \multicolumn{1}{c}{\textit{\textbf{{\tool}}}}
  \\ \midrule
  \multirow{5}{*}{KI} &
\multirow{1}{*}{{GPT-3.5}} &
 
  \multicolumn{1}{c}{19.7\%} &
  \multicolumn{1}{c}{\textbf{33.7\%}} &
  \multicolumn{1}{c}{30.2\%} &
  \multicolumn{1}{c}{31.6\%} &
  &
   \multicolumn{1}{c}{9.3\%} &
  \multicolumn{1}{c}{19.0\%} &
  \multicolumn{1}{c}{19.9\%} &
  \multicolumn{1}{c}{\textbf{23.9\%}}
  
  \\ 

\cline{2-11}
\rule{0pt}{2.6ex}
  &
   \multirow{1}{*}{{GPT-4}} &
 
   \multicolumn{1}{c}{37.9\%} &
  \multicolumn{1}{c}{41.5\%} &
  \multicolumn{1}{c}{40.5\%} &
  \multicolumn{1}{c}{\textbf{43.0\%}} &
  &
   \multicolumn{1}{c}{30.8\%} &
  \multicolumn{1}{c}{32.3\%} &
  \multicolumn{1}{c}{32.1\%} &
  \multicolumn{1}{c}{\textbf{36.0\%}}
  
  \\ 
   \cline{2-11}
   \rule{0pt}{2.6ex}
    &
\multirow{1}{*}{{Llama2-13B}} &

   \multicolumn{1}{c}{8.3\%} &
  \multicolumn{1}{c}{29.7\%} &
  \multicolumn{1}{c}{28.6\%} &
  \multicolumn{1}{c}{\textbf{32.9\%}} &
  &
   \multicolumn{1}{c}{1.8\%} &
  \multicolumn{1}{c}{16.7\%} &
  \multicolumn{1}{c}{15.8\%} &
  \multicolumn{1}{c}{\textbf{21.1\%}}
  
  \\ 

 

  \cline{2-11}
  \rule{0pt}{2.6ex}
   &
\multirow{1}{*}{{Llama3-70B}} &

   \multicolumn{1}{c}{27.0\%} &
  \multicolumn{1}{c}{32.9\%} &
  \multicolumn{1}{c}{32.4\%} &
  \multicolumn{1}{c}{\textbf{35.6\%}} &
  &
   \multicolumn{1}{c}{4.6\%} &
  \multicolumn{1}{c}{19.9\%} &
  \multicolumn{1}{c}{19.2\%} &
  \multicolumn{1}{c}{\textbf{22.7\%}}
  
  \\ 
   \cline{2-11}
   \rule{0pt}{2.6ex}
    &
\multirow{1}{*}{{Qwen2.5-32B}} &

   \multicolumn{1}{c}{17.9\%} &
  \multicolumn{1}{c}{\textbf{35.7\%}} &
  \multicolumn{1}{c}{30.6\%} &
  \multicolumn{1}{c}{31.6\%} &
  &
   \multicolumn{1}{c}{4.2\%} &
  \multicolumn{1}{c}{\textbf{23.1\%}} &
  \multicolumn{1}{c}{20.7\%} &
  \multicolumn{1}{c}{21.1\%}
  \\

\midrule
 \multirow{5}{*}{KC} &
\multirow{1}{*}{{GPT-3.5}} &
 
  \multicolumn{1}{c}{19.7\%} &
  \multicolumn{1}{c}{33.7\%} &
  \multicolumn{1}{c}{68.1\%} &
  \multicolumn{1}{c}{\textbf{76.0\%}} &
  &
   \multicolumn{1}{c}{9.3\%} &
  \multicolumn{1}{c}{19.0\%} &
  \multicolumn{1}{c}{54.6\%} &
  \multicolumn{1}{c}{\textbf{81.5\%}}
  
  \\ 

\cline{2-11}
\rule{0pt}{2.6ex}
  &
   \multirow{1}{*}{{GPT-4}} &
 
   \multicolumn{1}{c}{37.9\%} &
  \multicolumn{1}{c}{41.5\%} &
  \multicolumn{1}{c}{72.9\%} &
  \multicolumn{1}{c}{\textbf{82.6\%}} &
  &
   \multicolumn{1}{c}{30.8\%} &
  \multicolumn{1}{c}{32.3\%} &
  \multicolumn{1}{c}{59.3\%} &
  \multicolumn{1}{c}{\textbf{88.6\%}}
  
  \\ 
   \cline{2-11}
   \rule{0pt}{2.6ex}
    &
\multirow{1}{*}{{Llama2-13B}} &

   \multicolumn{1}{c}{8.3\%} &
  \multicolumn{1}{c}{29.7\%} &
  \multicolumn{1}{c}{64.4\%} &
  \multicolumn{1}{c}{\textbf{74.1\%}} &
  &
   \multicolumn{1}{c}{1.8\%} &
  \multicolumn{1}{c}{16.7\%} &
  \multicolumn{1}{c}{51.7\%} &
  \multicolumn{1}{c}{\textbf{74.0\%}}
  
  \\ 

 

  \cline{2-11}
  \rule{0pt}{2.6ex}
   &
\multirow{1}{*}{{Llama3-70B}} &

   \multicolumn{1}{c}{27.0\%} &
  \multicolumn{1}{c}{32.9\%} &
  \multicolumn{1}{c}{67.8\%} &
  \multicolumn{1}{c}{\textbf{79.5\%}} &
  &
   \multicolumn{1}{c}{4.6\%} &
  \multicolumn{1}{c}{19.9\%} &
  \multicolumn{1}{c}{49.4\%} &
  \multicolumn{1}{c}{\textbf{80.0\%}}
  
  \\ 
   \cline{2-11}
   \rule{0pt}{2.6ex}
    &
\multirow{1}{*}{{Qwen2.5-32B}} &

   \multicolumn{1}{c}{17.9\%} &
  \multicolumn{1}{c}{35.7\%} &
  \multicolumn{1}{c}{63.8\%} &
  \multicolumn{1}{c}{\textbf{77.0\%}} &
  &
   \multicolumn{1}{c}{4.2\%} &
  \multicolumn{1}{c}{23.1\%} &
  \multicolumn{1}{c}{49.4\%} &
  \multicolumn{1}{c}{\textbf{83.8\%}}
  \\

\bottomrule
\end{tabular}

        \end{threeparttable}
}
\end{table}

==> tab/pre_experiment.tex <==
\begin{table}[t]
  \caption{The response accuracy (ACC) of LLM under complete and incomplete chain of evidence. }
  \label{tab:pre_acc}
  
\resizebox{0.5\textwidth }{!}{
\begin{threeparttable}
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{\textbf{Metric}} &
  

  \multicolumn{2}{c}{\textbf{HotpotQA}} & &
  \multicolumn{2}{c}{\textbf{2WikiMultihopQA}}
  \\    \cline{2-3} \cline{5-6} 


     
   &

   


  \multicolumn{1}{c}{\textit{\textbf{Complete}}} &
  \multicolumn{1}{c}{\textit{\textbf{Incomplete}}} & 
  &
  \multicolumn{1}{c}{\textit{\textbf{Complete}}} &
  \multicolumn{1}{c}{\textit{\textbf{Incomplete}}}
  \\ \midrule
\multirow{1}{*}{{ACC}} &
 
  
  \multicolumn{1}{c}{91.9\%} &
  \multicolumn{1}{c}{81.7\%} &
  &
  \multicolumn{1}{c}{96.8\%} &
  \multicolumn{1}{c}{81.1\%}
  \\ 



\bottomrule
\end{tabular}

        \end{threeparttable}
}
\end{table}

==> tab/test.tex <==

 
 \multirow{6}{*}{HotpotQA} & GPT-3.5 & 59.0/33.0  & 61.0/25.0 & \textbf{46.0/52.0} & 78.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & GPT-4 & 79.0/10.0 & 74.0/13.0 &  \textbf{63.0/28.0} & 78.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & GPT-4o & 72.0/11.0 & 78.0/10.0 &  \textbf{52.0/40.0} & 79.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Llama3-8B & 70.0/15.0 & 52.0/31.0 &  \textbf{46.0/48.0} & 70.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Llama3-70B & 72.0/17.0 & 76.0/8.0 &  \textbf{51.0/45.0} & 83.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Deepseek-V3-0324 & 78.0/8.0 & 71.0/15.0 & \textbf{60.0/34.0} & 75.0  \\

\noalign{\vspace{3pt}} \cline{1-6}\noalign{\vspace{3pt}} 
 \multirow{6}{*}{MS-MARCO} & GPT-3.5 & 73.0/14.0 & 81.0/12.0 &  \textbf{56.0/30.0} & 82.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & GPT-4 & 88.0/5.0 & 85.0/8.0 & \textbf{57.0/34.0} & 89.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & GPT-4o & 86.0/4.0 & 84.0/8.0 & \textbf{67.0/28.0} & 87.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Llama3-8B & 83.0/11.0 & 73.0/23.0 & \textbf{60.0/35.0} & 91.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Llama3-70B & 86.0/9.0 & 58.0/39.0 & \textbf{56.0/37.0} & 91.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Deepseek-V3-0324 & 88.0/5.0 & 85.0/10.0 & \textbf{82.0/11.0} & 89.0  \\

\noalign{\vspace{3pt}} \cline{1-6}\noalign{\vspace{3pt}} 
  \multirow{6}{*}{NQ} & GPT-3.5 & 62.0/21.0  & 75.0/9.0 & \textbf{44.0/47.0} & 71.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & GPT-4 & 81.0/5.0 & 83.0/7.0 & \textbf{69.0/23.0} & 80.0  \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & GPT-4o & 80.0/8.0 & 82.0/9.0 & \textbf{71.0/23.0} & 84.0 \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Llama3-8B & 78.0/9.0 & 69.0/17.0 & \textbf{60.0/33.0} & 78.0 \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Llama3-70B & 83.0/5.0 & 87.0/5.0 & \textbf{58.0/38.0} & 86.0 \\
\noalign{\vspace{3pt}} \cline{2-6}\noalign{\vspace{3pt}} 
 & Deepseek-V3-0324 & 86.0/0.0 & 84.0/6.0 & \textbf{75.0/11.0} & 86.0 \\
